Observation of muon neutrino disappearance with the MINOS detectors and the NuMI neutrino beam

This letter reports results from the MINOS experiment based on its initial exposure to neutrinos from the Fermilab NuMI beam. The rate and energy spectra of charged current muon neutrino interactions are compared in two detectors located along the beam axis at distances of 1 km and 735 km. With 1.27 x 10^{20} 120 GeV protons incident on the NuMI target, 215 events with energies below 30 GeV are observed at the Far Detector, compared to an expectation of 336 \pm 14.4 events. The data are consistent with muon neutrino disappearance via oscillation with |\Delta m^2_{23}| = 2.74^{+0.44}_{-0.26} x 10^{-3} eV^2/c^4 and sin^2(2\theta_{23}) > 0.87 (at 60% C.L.).

==> CC-authors.tex <==

\title{Observation of muon neutrino disappearance with the MINOS detectors in the NuMI neutrino beam}

\newcommand{\Cambridge}{Cavendish Laboratory, Univ. of Cambridge, Madingley Road, Cambridge CB3 0HE, UK}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL 60510}
\newcommand{\RAL}{Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}
\newcommand{\UCL}{Dept. of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, UK}
\newcommand{\Caltech}{Lauritsen Lab, California Institute of Technology, Pasadena, CA 91125}
\newcommand{\ANL}{Argonne National Laboratory, Argonne, IL 60439}
\newcommand{\Athens}{Department of Physics, University of Athens, GR-15771 Athens, Greece}
\newcommand{\NTUAthens}{Dept. of Physics, National Tech. Univ. of Athens, GR-15780 Athens, Greece}
\newcommand{\Benedictine}{Physics Dept., Benedictine University, Lisle, IL 60532}
\newcommand{\BIMC}{Dept. of Rad. Oncology, Beth Israel Med. Center, New York, NY 10003}
\newcommand{\BNL}{Brookhaven National Laboratory, Upton, NY 11973}
\newcommand{\Beijing}{Inst. of High Energy Physics, Chinese Academy of Sciences, Beijing 100039, China}
\newcommand{\CdF}{APC -- Coll\`{e}ge de France, 11 Place Marcelin Berthelot, F-75231 Paris Cedex 05, France}
\newcommand{\Cleveland}{Cleveland Clinic, Cleveland, OH 44195}
\newcommand{\Columbia}{Physics Department, Columbia University, New York, NY 10027}
\newcommand{\GEHealth}{GE Healthcare, Florence SC 29501}
\newcommand{\DOE}{Div. of High Energy Physics, U.S. Dept. of Energy, Germantown, MD 20874}
\newcommand{\Harvard}{Dept. of Physics, Harvard University, Cambridge, MA 02138}
\newcommand{\HolyCross}{Holy Cross College, Notre Dame, IN 46556}
\newcommand{\IIT}{Physics Division, Illinois Institute of Technology, Chicago, IL 60616}
\newcommand{\Indiana}{Physics Department, Indiana University, Bloomington, IN 47405}
\newcommand{\ITEP}{High Energy Exp. Physics Dept., Inst. of Theor. and Exp. Physics, 
  B. Cheremushkinskaya, 25, 117218 Moscow, Russia}
\newcommand{\JMU}{Physics Dept., James Madison University, Harrisonburg, VA 22807}
\newcommand{\JINR}{Joint Inst. for Nucl. Research, Dubna, Moscow Region, RU-141980, Russia}
\newcommand{\LASL}{Nucl. Nonprolif. Div., Threat Reduc. Dir., Los Alamos National Laboratory, Los Alamos, NM 87545}
\newcommand{\LBL}{Physics Div., Lawrence Berkeley National Laboratory, Berkeley, CA 94720}
\newcommand{\Lebedev}{Nuclear Physics Dept., Lebedev Physical Inst., Leninsky Prospect 53, 117924 Moscow, Russia}
\newcommand{\LLL}{Lawrence Livermore National Laboratory, Livermore, CA 94550}
\newcommand{\MIT}{Lincoln Laboratory, Massachusetts Institute of Technology, Lexington, MA 02420}
\newcommand{\Minnesota}{University of Minnesota, Minneapolis, MN 55455}
\newcommand{\Crookston}{Math, Science and Technology Dept., Univ. of Minnesota -- Crookston, Crookston, MN 56716}
\newcommand{\Duluth}{Dept. of Physics, Univ. of Minnesota -- Duluth, Duluth, MN 55812}
\newcommand{\Oxford}{Sub-dept. of Particle Physics, Univ. of Oxford,  Denys Wilkinson Bldg, Keble Road, Oxford OX1 3RH, UK}
\newcommand{\PSU}{Dept. of Physics, Pennsylvania State Univ., University Park, PA 16802}
\newcommand{\Pittsburgh}{Dept. of Physics and Astronomy, Univ. of Pittsburgh, Pittsburgh, PA 15260}
\newcommand{\IHEP}{Inst. for High Energy Physics, Protvino, Moscow Region RU-140284, Russia}
\newcommand{\RoyalH}{Physics Dept., Royal Holloway, Univ. of London, Egham, Surrey, TW20 0EX, UK}
\newcommand{\Carolina}{Dept. of Physics and Astronomy, Univ. of South Carolina, Columbia, SC 29208}
\newcommand{\SLAC}{Stanford Linear Accelerator Center, Stanford, CA 94309}
\newcommand{\Stanford}{Department of Physics, Stanford University, Stanford, CA 94305}
\newcommand{\Sussex}{Dept. of Physics and Astronomy, University of Sussex, Falmer, Brighton BN1 9QH, UK}
\newcommand{\TexasAM}{Physics Dept., Texas A\&M Univ., College Station, TX 77843}
\newcommand{\Texas}{Dept. of Physics, Univ. of Texas, 1 University Station, Austin, TX 78712}
\newcommand{\TechX}{Tech-X Corp, Boulder, CO 80303}
\newcommand{\Tufts}{Physics Dept., Tufts University, Medford, MA 02155}
\newcommand{\UNICAMP}{Univ. Estadual de Campinas, IF-UNICAMP, CP 6165, 13083-970, Campinas, SP, Brazil}
\newcommand{\USP}{Inst. de F\'{i}sica, Univ. de S\~{a}o Paulo,  CP 66318, 05315-970, S\~{a}o Paulo, SP, Brazil}
\newcommand{\Washington}{Physics Dept., Western Washington Univ., Bellingham, WA 98225}
\newcommand{\WandM}{Dept. of Physics, College of William \& Mary, Williamsburg, VA 23187}
\newcommand{\Wisconsin}{Physics Dept., Univ. of Wisconsin, Madison, WI 53706}
\newcommand{\deceased}{Deceased.}

\affiliation{\ANL}
\affiliation{\Athens}
\affiliation{\Benedictine}
\affiliation{\BNL}
\affiliation{\Caltech}
\affiliation{\Cambridge}
\affiliation{\UNICAMP}
\affiliation{\Beijing}
\affiliation{\CdF}
\affiliation{\Columbia}
\affiliation{\FNAL}
\affiliation{\Harvard}
\affiliation{\IIT}
\affiliation{\Indiana}
\affiliation{\IHEP}
\affiliation{\ITEP}
\affiliation{\JMU}
\affiliation{\JINR}
\affiliation{\Lebedev}
\affiliation{\LLL}
\affiliation{\UCL}
\affiliation{\Minnesota}
\affiliation{\Duluth}
\affiliation{\Oxford}
\affiliation{\Pittsburgh}
\affiliation{\RAL}
\affiliation{\USP}
\affiliation{\Carolina}
\affiliation{\Stanford}
\affiliation{\Sussex}
\affiliation{\TexasAM}
\affiliation{\Texas}
\affiliation{\Tufts}
\affiliation{\Washington}
\affiliation{\WandM}
\affiliation{\Wisconsin}

\author{D.~G.~Michael}
\altaffiliation{\deceased}
\affiliation{\Caltech}

\author{P.~Adamson}
\affiliation{\FNAL}
\affiliation{\UCL}
\affiliation{\Sussex}

\author{T.~Alexopoulos}
%\altaffiliation[Now at\ ]{\NTUAthens .}
\affiliation{\Wisconsin}

\author{W.~W.~M.~Allison}
\affiliation{\Oxford}

\author{G.~J.~Alner}
\affiliation{\RAL}

\author{K.~Anderson}
\affiliation{\FNAL}

\author{C.~Andreopoulos}
\affiliation{\RAL}
\affiliation{\Athens}

\author{M.~Andrews}
\affiliation{\FNAL}

\author{R.~Andrews}
\affiliation{\FNAL}

\author{K.~E.~Arms}
\affiliation{\Minnesota}

\author{R.~Armstrong}
\affiliation{\Indiana}

\author{C.~Arroyo}
\affiliation{\Stanford}

\author{D.~J.~Auty}
\affiliation{\Sussex}

\author{S.~Avvakumov}
\affiliation{\Stanford}

\author{D.~S.~Ayres}
\affiliation{\ANL}

\author{B.~Baller}
\affiliation{\FNAL}

\author{B.~Barish}
\affiliation{\Caltech}

\author{M.~A.~Barker}
\affiliation{\Oxford}

\author{P.~D.~Barnes~Jr.}
\affiliation{\LLL}

\author{G.~Barr}
\affiliation{\Oxford}

\author{W.~L.~Barrett}
\affiliation{\Washington}

\author{E.~Beall}
%\altaffiliation[Now at\ ]{\Cleveland .}
\affiliation{\ANL}
\affiliation{\Minnesota}

\author{B.~R.~Becker}
\affiliation{\Minnesota}

\author{A.~Belias}
\affiliation{\RAL}

\author{T.~Bergfeld}
%\altaffiliation[Now at\ ]{\GEHealth .}
\affiliation{\Carolina}

\author{R.~H.~Bernstein}
\affiliation{\FNAL}

\author{D.~Bhattacharya}
\affiliation{\Pittsburgh}

\author{M.~Bishai}
\affiliation{\BNL}

\author{A.~Blake}
\affiliation{\Cambridge}

\author{V.~Bocean}
\affiliation{\FNAL}

\author{B.~Bock}
\affiliation{\Duluth}

\author{G.~J.~Bock}
\affiliation{\FNAL}

\author{J.~Boehm}
\affiliation{\Harvard}

\author{D.~J.~Boehnlein}
\affiliation{\FNAL}

\author{D.~Bogert}
\affiliation{\FNAL}

\author{P.~M.~Border}
\affiliation{\Minnesota}

\author{C.~Bower}
\affiliation{\Indiana}

\author{S.~Boyd}
\affiliation{\Pittsburgh}

\author{E.~Buckley-Geer}
\affiliation{\FNAL}

\author{C.~Bungau}
\affiliation{\Sussex}

\author{A.~Byon-Wagner}
%\altaffiliation[Now at\ ]{\DOE .}
\affiliation{\FNAL}

\author{A.~Cabrera}
%\altaffiliation[Now at\ ]{\CdF .}
\affiliation{\Oxford}

\author{J.~D.~Chapman}
\affiliation{\Cambridge}

\author{T.~R.~Chase}
\affiliation{\Minnesota}

\author{D.~Cherdack}
\affiliation{\Tufts}

\author{S.~K.~Chernichenko}
\affiliation{\IHEP}

\author{S.~Childress}
\affiliation{\FNAL}

\author{B.~C.~Choudhary}
\affiliation{\FNAL}
\affiliation{\Caltech}

\author{J.~H.~Cobb}
\affiliation{\Oxford}

\author{J.~D.~Cossairt}
\affiliation{\FNAL}

\author{H.~Courant}
\affiliation{\Minnesota}

\author{D.~A.~Crane}
\affiliation{\ANL}

\author{A.~J.~Culling}
\affiliation{\Cambridge}

\author{J.~W.~Dawson}
\affiliation{\ANL}

\author{J.~K.~de~Jong}
\affiliation{\IIT}

\author{D.~M.~DeMuth}
%\altaffiliation[Now at\ ]{\Crookston .}
\affiliation{\Minnesota}

\author{A.~De~Santo}
%\altaffiliation[Now at\ ]{\RoyalH .}
\affiliation{\Oxford}

\author{M.~Dierckxsens}
\affiliation{\BNL}

\author{M.~V.~Diwan}
\affiliation{\BNL}

\author{M.~Dorman}
\affiliation{\UCL}
\affiliation{\RAL}

\author{G.~Drake}
\affiliation{\ANL}

\author{D.~Drakoulakos}
\affiliation{\Athens}

\author{R.~Ducar}
\affiliation{\FNAL}

\author{T.~Durkin}
\affiliation{\RAL}

\author{A.~R.~Erwin}
\affiliation{\Wisconsin}

\author{C.~O.~Escobar}
\affiliation{\UNICAMP}

\author{J.~J.~Evans}
\affiliation{\Oxford}

\author{O.~D.~Fackler}
\affiliation{\LLL}

\author{E.~Falk~Harris}
\affiliation{\Sussex}

\author{G.~J.~Feldman}
\affiliation{\Harvard}

\author{N.~Felt}
\affiliation{\Harvard}

\author{T.~H.~Fields}
\affiliation{\ANL}

\author{R.~Ford}
\affiliation{\FNAL}

\author{M.~V.~Frohne}
%\altaffiliation[Now at\ ]{\HolyCross .}
\affiliation{\Benedictine}

\author{H.~R.~Gallagher}
\affiliation{\Tufts}
\affiliation{\Oxford}
\affiliation{\ANL}
\affiliation{\Minnesota}

\author{M.~Gebhard}
\affiliation{\Indiana}

\author{G.~A.~Giurgiu}
\affiliation{\ANL}

\author{A.~Godley}
\affiliation{\Carolina}

\author{J.~Gogos}
\affiliation{\Minnesota}

\author{M.~C.~Goodman}
\affiliation{\ANL}

\author{Yu.~Gornushkin}
\affiliation{\JINR}

\author{P.~Gouffon}
\affiliation{\USP}

\author{R.~Gran}
\affiliation{\Duluth}

\author{E.~Grashorn}
\affiliation{\Minnesota}
\affiliation{\Duluth}

\author{N.~Grossman}
\affiliation{\FNAL}

\author{J.~J.~Grudzinski}
\affiliation{\ANL}

\author{K.~Grzelak}
\affiliation{\Oxford}

\author{V.~Guarino}
\affiliation{\ANL}

\author{A.~Habig}
\affiliation{\Duluth}

\author{R.~Halsall}
\affiliation{\RAL}

\author{J.~Hanson}
\affiliation{\Caltech}

\author{D.~Harris}
\affiliation{\FNAL}

\author{P.~G.~Harris}
\affiliation{\Sussex}

\author{J.~Hartnell}
\affiliation{\RAL}
\affiliation{\Oxford}

\author{E.~P.~Hartouni}
\affiliation{\LLL}

\author{R.~Hatcher}
\affiliation{\FNAL}

\author{K.~Heller}
\affiliation{\Minnesota}

\author{N.~Hill}
\affiliation{\ANL}

\author{Y.~Ho}
%\altaffiliation[Now at\ ]{\BIMC .}
\affiliation{\Columbia}

\author{A.~Holin}
\affiliation{\UCL}

\author{C.~Howcroft}
\affiliation{\Caltech}
\affiliation{\Cambridge}

\author{J.~Hylen}
\affiliation{\FNAL}

\author{M.~Ignatenko}
\affiliation{\JINR}

\author{D.~Indurthy}
\affiliation{\Texas}

\author{G.~M.~Irwin}
\affiliation{\Stanford}

\author{M.~Ishitsuka}
\affiliation{\Indiana}

\author{D.~E.~Jaffe}
\affiliation{\Harvard}

\author{C.~James}
\affiliation{\FNAL}

\author{L.~Jenner}
\affiliation{\UCL}

\author{D.~Jensen}
\affiliation{\FNAL}

\author{T.~Joffe-Minor}
\affiliation{\ANL}

\author{T.~Kafka}
\affiliation{\Tufts}

\author{H.~J.~Kang}
\affiliation{\Stanford}

\author{S.~M.~S.~Kasahara}
\affiliation{\Minnesota}

\author{J.~Kilmer}
\affiliation{\FNAL}

\author{H.~Kim}
\affiliation{\Caltech}

\author{M.~S.~Kim}
\affiliation{\Pittsburgh}

\author{G.~Koizumi}
\affiliation{\FNAL}

\author{S.~Kopp}
\affiliation{\Texas}

\author{M.~Kordosky}
\affiliation{\UCL}
\affiliation{\Texas}

\author{D.~J.~Koskinen}
\affiliation{\UCL}
\affiliation{\Duluth}

\author{M.~Kostin}
%\altaffiliation[Now at\ ]{\FNAL .}
\affiliation{\Texas}

\author{S.K.~Kotelnikov}
\affiliation{\Lebedev}

\author{D.~A.~Krakauer}
\affiliation{\ANL}

\author{A.~Kreymer}
\affiliation{\FNAL}

\author{S.~Kumaratunga}
\affiliation{\Minnesota}

\author{A.~S.~Ladran}
\affiliation{\LLL}

\author{K.~Lang}
\affiliation{\Texas}

\author{C.~Laughton}
\affiliation{\FNAL}

\author{A.~Lebedev}
\affiliation{\Harvard}

\author{R.~Lee}
%\altaffiliation[Now at\ ]{\MIT .}
\affiliation{\Harvard}

\author{W.~Y.~Lee}
%\altaffiliation[Now at\ ]{\LBL .}
\affiliation{\Columbia}

\author{M.~A.~Libkind}
\affiliation{\LLL}

\author{J.~Ling}
\affiliation{\Carolina}

\author{J.~Liu}
\affiliation{\Texas}

\author{P.~J.~Litchfield}
\affiliation{\Minnesota}
\affiliation{\RAL}

\author{R.~P.~Litchfield}
\affiliation{\Oxford}

\author{N.~P.~Longley}
\affiliation{\Minnesota}

\author{P.~Lucas}
\affiliation{\FNAL}

\author{W.~Luebke}
\affiliation{\IIT}

\author{S.~Madani}
\affiliation{\RAL}

\author{E.~Maher}
\affiliation{\Minnesota}

\author{V.~Makeev}
\affiliation{\FNAL}
\affiliation{\IHEP}

\author{W.~A.~Mann}
\affiliation{\Tufts}

\author{A.~Marchionni}
\affiliation{\FNAL}

\author{A.~D.~Marino}
\affiliation{\FNAL}

\author{M.~L.~Marshak}
\affiliation{\Minnesota}

\author{J.~S.~Marshall}
\affiliation{\Cambridge}

\author{N.~Mayer}
\affiliation{\Duluth}

\author{J.~McDonald}
\affiliation{\Pittsburgh}

\author{A.~M.~McGowan}
\affiliation{\ANL}
\affiliation{\Minnesota}

\author{J.~R.~Meier}
\affiliation{\Minnesota}

\author{G.~I.~Merzon}
\affiliation{\Lebedev}

\author{M.~D.~Messier}
\affiliation{\Indiana}
\affiliation{\Harvard}

\author{R.~H.~Milburn}
\affiliation{\Tufts}

\author{J.~L.~Miller}
\altaffiliation{\deceased}
\affiliation{\JMU}
\affiliation{\Indiana}

\author{W.~H.~Miller}
\affiliation{\Minnesota}

\author{S.~R.~Mishra}
\affiliation{\Carolina}
\affiliation{\Harvard}

\author{A.~Mislivec}
\affiliation{\Duluth}

\author{P.~S.~Miyagawa}
\affiliation{\Oxford}

\author{C.~D.~Moore}
\affiliation{\FNAL}

\author{J.~Morf\'{i}n}
\affiliation{\FNAL}

\author{R.~Morse}
\affiliation{\Sussex}

\author{L.~Mualem}
\affiliation{\Minnesota}

\author{S.~Mufson}
\affiliation{\Indiana}

\author{S.~Murgia}
\affiliation{\Stanford}

\author{M.~J.~Murtagh}
\altaffiliation{\deceased}
\affiliation{\BNL}

\author{J.~Musser}
\affiliation{\Indiana}

\author{D.~Naples}
\affiliation{\Pittsburgh}

\author{C.~Nelson}
\affiliation{\FNAL}

\author{J.~K.~Nelson}
\affiliation{\WandM}
\affiliation{\FNAL}
\affiliation{\Minnesota}

\author{H.~B.~Newman}
\affiliation{\Caltech}

\author{F.~Nezrick}
\affiliation{\FNAL}

\author{R.~J.~Nichol}
%\altaffiliation[Now at\ ]{\PSU .}
\affiliation{\UCL}

\author{T.~C.~Nicholls}
\affiliation{\RAL}

\author{J.~P.~Ochoa-Ricoux}
\affiliation{\Caltech}

\author{J.~Oliver}
\affiliation{\Harvard}

\author{W.~P.~Oliver}
\affiliation{\Tufts}

\author{V.~A.~Onuchin}
\affiliation{\IHEP}

\author{T.~Osiecki}
\affiliation{\Texas}

\author{R.~Ospanov}
\affiliation{\Texas}

\author{J.~Paley}
\affiliation{\Indiana}

\author{V.~Paolone}
\affiliation{\Pittsburgh}

\author{A.~Para}
\affiliation{\FNAL}

\author{T.~Patzak}
\affiliation{\CdF}
\affiliation{\Tufts}

\author{\v{Z}.~Pavlovi\'{c}}
\affiliation{\Texas}

\author{G.~F.~Pearce}
\affiliation{\RAL}

\author{N.~Pearson}
\affiliation{\Minnesota}

\author{C.~W.~Peck}
\affiliation{\Caltech}

\author{C.~Perry}
\affiliation{\Oxford}

\author{E.~A.~Peterson}
\affiliation{\Minnesota}

\author{D.~A.~Petyt}
\affiliation{\Minnesota}
\affiliation{\RAL}
\affiliation{\Oxford}

\author{H.~Ping}
\affiliation{\Wisconsin}

\author{R.~Piteira}
\affiliation{\CdF}

\author{R.~Pittam}
\affiliation{\Oxford}

\author{A.~Pla-Dalmau}
\affiliation{\FNAL}

\author{R.~K.~Plunkett}
\affiliation{\FNAL}

\author{L.~E.~Price}
\affiliation{\ANL}

\author{M.~Proga}
\affiliation{\Texas}

\author{D.~R.~Pushka}
\affiliation{\FNAL}

\author{D.~Rahman}
\affiliation{\Minnesota}

\author{R.~A.~Rameika}
\affiliation{\FNAL}

\author{T.~M.~Raufer}
\affiliation{\Oxford}

\author{A.~L.~Read}
\affiliation{\FNAL}

\author{B.~Rebel}
\affiliation{\FNAL}
\affiliation{\Indiana}

\author{J.~Reichenbacher}
\affiliation{\ANL}

\author{D.~E.~Reyna}
\affiliation{\ANL}

\author{C.~Rosenfeld}
\affiliation{\Carolina}

\author{H.~A.~Rubin}
\affiliation{\IIT}

\author{K.~Ruddick}
\affiliation{\Minnesota}

\author{V.~A.~Ryabov}
\affiliation{\Lebedev}

\author{R.~Saakyan}
\affiliation{\UCL}

\author{M.~C.~Sanchez}
\affiliation{\Harvard}
\affiliation{\Tufts}

\author{N.~Saoulidou}
\affiliation{\FNAL}
\affiliation{\Athens}

\author{J.~Schneps}
\affiliation{\Tufts}

\author{P.~V.~Schoessow}
%\altaffiliation[Now at\ ]{\TechX .}
\affiliation{\ANL}

\author{P.~Schreiner}
\affiliation{\Benedictine}

\author{R.~Schwienhorst}
\affiliation{\Minnesota}

\author{V.~K.~Semenov}
\affiliation{\IHEP}

\author{S.-M.~Seun}
\affiliation{\Harvard}

\author{P.~Shanahan}
\affiliation{\FNAL}

\author{P.~D.~Shield}
\affiliation{\Oxford}

\author{W.~Smart}
\affiliation{\FNAL}

\author{V.~Smirnitsky}
\affiliation{\ITEP}

\author{C.~Smith}
\affiliation{\UCL}
\affiliation{\Sussex}
\affiliation{\Caltech}

\author{P.~N.~Smith}
\affiliation{\Sussex}

\author{A.~Sousa}
\affiliation{\Oxford}
\affiliation{\Tufts}

\author{B.~Speakman}
\affiliation{\Minnesota}

\author{P.~Stamoulis}
\affiliation{\Athens}

\author{A.~Stefanik}
\affiliation{\FNAL}

\author{P.~Sullivan}
\affiliation{\Oxford}

\author{J.~M.~Swan}
\affiliation{\LLL}

\author{P.~A.~Symes}
\affiliation{\Sussex}

\author{N.~Tagg}
\affiliation{\Tufts}
\affiliation{\Oxford}

\author{R.~L.~Talaga}
\affiliation{\ANL}

\author{E.~Tetteh-Lartey}
\affiliation{\TexasAM}

\author{J.~Thomas}
\affiliation{\UCL}
\affiliation{\Oxford}
\affiliation{\FNAL}

\author{J.~Thompson}
\altaffiliation{\deceased}
\affiliation{\Pittsburgh}

\author{M.~A.~Thomson}
\affiliation{\Cambridge}

\author{J.~L.~Thron}
%\altaffiliation[Now at\ ]{\LASL .}
\affiliation{\ANL}

\author{G.~Tinti}
\affiliation{\Oxford}

\author{R.~Trendler}
\affiliation{\FNAL}

\author{J.~Trevor}
\affiliation{\Caltech}

\author{I.~Trostin}
\affiliation{\ITEP}

\author{V.~A.~Tsarev}
\affiliation{\Lebedev}

\author{G.~Tzanakos}
\affiliation{\Athens}

\author{J.~Urheim}
\affiliation{\Indiana}
\affiliation{\Minnesota}

\author{P.~Vahle}
\affiliation{\UCL}
\affiliation{\Texas}

\author{M.~Vakili}
\affiliation{\TexasAM}

\author{K.~Vaziri}
\affiliation{\FNAL}

\author{C.~Velissaris}
\affiliation{\Wisconsin}

\author{V.~Verebryusov}
\affiliation{\ITEP}

\author{B.~Viren}
\affiliation{\BNL}

\author{L.~Wai}
%\altaffiliation[Now at\ ]{\SLAC .}
\affiliation{\Stanford}

\author{C.~P.~Ward}
\affiliation{\Cambridge}

\author{D.~R.~Ward}
\affiliation{\Cambridge}

\author{M.~Watabe}
\affiliation{\TexasAM}

\author{A.~Weber}
\affiliation{\Oxford}
\affiliation{\RAL}

\author{R.~C.~Webb}
\affiliation{\TexasAM}

\author{A.~Wehmann}
\affiliation{\FNAL}

\author{N.~West}
\affiliation{\Oxford}

\author{C.~White}
\affiliation{\IIT}

\author{R.~F.~White}
\affiliation{\Sussex}

\author{S.~G.~Wojcicki}
\affiliation{\Stanford}

\author{D.~M.~Wright}
\affiliation{\LLL}

\author{Q.~K.~Wu}
\affiliation{\Carolina}

\author{W.~G.~Yan}
\affiliation{\Beijing}

\author{T.~Yang}
\affiliation{\Stanford}

\author{F.~X.~Yumiceva}
\affiliation{\WandM}

\author{J.~C.~Yun}
\affiliation{\FNAL}

\author{H.~Zheng}
\affiliation{\Caltech}

\author{M.~Zois}
\affiliation{\Athens}

\author{R.~Zwaska}
\affiliation{\FNAL}
\affiliation{\Texas}

\collaboration{The MINOS Collaboration}
\noaffiliation

\date{\today}


